Deep-Graph-Sprints: Accelerated Representation Learning in Continuous-Time Dynamic Graphs

Continuous-time dynamic graphs (CTDGs) are essential for modeling interconnected, evolving systems. Traditional methods for extracting knowledge from these graphs often depend on feature engineering or deep learning. Feature engineering is limited by the manual and time-intensive nature of crafting features, while deep learning approaches suffer from high inference latency, making them impractical for real-time applications. This paper introduces Deep-Graph-Sprints (DGS), a novel deep learning architecture designed for efficient representation learning on CTDGs with low-latency inference requirements. We benchmark DGS against state-of-the-art (SOTA) feature engineering and graph neural network methods using five diverse datasets. The results indicate that DGS achieves competitive performance while inference speed improves between 4x and 12x compared to other deep learning approaches on our benchmark datasets. Our method effectively bridges the gap between deep representation learning and low-latency application requirements for CTDGs.

==> 2-related_work.tex <==

\section{Related Work}
\label{dgs_related_work_long}
%* Only dynamic graph methods
%* RNN based
%* Async
%* GS
%\begin{itemize}
%    \item RW based: RW-based
%    \item RNN/GNN based: ((TGN, Jodie, TGAT, Dyrep)): mention the AD modes and their limitations
%    \item Low latency:  (APAN, GS, HashGNN, SGSketch, ): mention the AD modes and their limitations
    
%\end{itemize}



Graph representation learning is crucial in transforming complex graph structures into usable formats for ML models. This section discusses the evolution of existing algorithms. While not all of these methods are directly used in our work, understanding their limitations and strengths has informed the development of our method.


\subsection{Random-walk Based Techniques}
A \emph{random-walk}, in the context of graph theory, is a stochastic process that derives random paths originating from a designated node. By conducting \emph{numerous} such walks, one can approximate the inherent structure of the network. Notably, if two nodes exhibit similar random-walks, it might suggest they occupy analogous structural roles in the network.

Traditional random-walk methods like, \textit{DeepWalk}~\cite{perozzi2014deepwalk}, LINE~\cite{tang2015line}, \textit{Node2vec}~\cite{grover2016node2vec},  \textit{Struc2vec}~\cite{ribeiro2017struc2vec}, \textit{Metapath2vec}~\cite{dong2017metapath2vec},
\textit{Role2vec}~\cite{ahmed2019role2vec}, are genuinely stochastic, choosing a random neighbor to progress the walk at each hop. \textit{Node2vec}~\cite{grover2016node2vec}, however, introduces a degree of bias, using two parameters, to direct the walks to be either shallower or deeper.

\cite{sajjad2019efficient} adapted random-walk techniques to DTDG. While this adaptation introduced a degree of efficiency, it remains constrained in its applicability, especially for CTDGs and in low-latency situations. In contrast, Node2bits~\cite{jin2019node2bits} integrates time-related details by separating the random walks it samples into different time windows. It combines node attributes into histograms during these times. \textit{Node2bits} creates binary representations to reduce memory footprint. These methods demand considerable computational resources for executing walks, making them less suitable for scenarios requiring low latency.



Further developments, such as continuous-time dynamic node embeddings (\textit{CTDNE})~\cite{lee2020dynamic,nguyen2018continuous}, were introduced to provide time-aware embeddings, augmenting the \textit{Node2vec}~\cite{grover2016node2vec} paradigm for CTDGs. These methodologies treat the graph as a stream of edges and perform temporal walks from seed nodes chosen through a temporally-biased distribution. Hyperbolic spaces have seen the application of temporal random-walks for embedding extraction~\cite{wang2021hyperbolic}. 


Moreover, the anonymous walks approach~\cite{wang2021inductive} employs causal anonymized walks to encode motif-centric data (motifs refer to subgraphs that occur within a real network at a frequency higher than what statistical probability would typically predict~\cite{ribeiro2021survey}). In parallel, \textit{NeurTWs}~\cite{jin2022neural} integrate time into the anonymous walks via Neural Ordinary Differential Equations (NeuralODEs). It is essential to note that these methods necessitate exhaustive random-walk executions.


A major limitation of random-walk-based approaches is their time complexity. To address efficiency, methods like \textit{B\_LIN}~\cite{tong2006fast} have been developed. This method improves efficiency by leveraging two prevalent characteristics found in many real-world graphs, namely, linear correlations and community-like structures.

Apart from time complexity, random-walks also impose significant demands on main memory volume. This issue is particularly relevant as many high-speed random-walk algorithms assume the entire graph fits within the main memory, a challenge highlighted by~\cite{xia2019random}. To address this, various strategies have been developed for graph partitioning and clustering. Notable among these are \textit{METIS}~\cite{karypis1997metis}, and \textit{RWDISK}~\cite{sarkar2010fast}, which offer practical solutions for managing large-scale graphs efficiently.


Random-walks have applications in domains such as collaborative filtering, recommender systems, computer vision, and more. For a comprehensive review of random-walk-based applications and the challenges they pose, the reader is directed to \cite{xia2019random}.


\subsection{\textit{K}-hop Neighborhood Based Methods}

More recently, we see a surge in deep learning algorithms for graph representation learning. Several approaches leverage GNNs to learn functions that generate node embeddings~\cite{hamilton2017inductive,ying2018graph,yang2020multisage,zhu2020collective}. 

Most GNN-based methods require a $k$-hop neighborhood on which message-passing operations lead to node embeddings. To deal with CTDGs, a simple approach is to consider a series of discrete snapshots of the graph over time, on which static methods are applied. Such approaches however do not take time properly into account and several works propose techniques to alleviate this issue~\cite{sankar2020dysat,goyal2018dyngem,jin2022generalizing}. To better deal with CTDGs, other works focus on including time-aware features or inductive biases into the architecture. \textit{DeepCoevolve}~\cite{dai2016deep} and \textit{Jodie}~\cite{kumar2019predicting} train two RNNs for bipartite graphs, one for each node type. Importantly, the previous hidden state of one RNN is also added as an input to the other RNN. In this way, the two RNNs interact, in essence performing single-hop graph aggregations. \textit{TGAT}~\cite{xu2020inductive} proposes to include temporal information in the form of time encodings, while \textit{TGN}~\cite{tgn_icml_grl2020} extends this framework and also includes a memory module taking the form of an RNN.  In~\cite{jin2020static}, the authors replace the discrete-time recurrent network of \textit{TGN} with a \textit{NeuralODE} modeling the continuous dynamics of node embeddings. 



GNNs are instrumental in analyzing vast time series data, but adapting them to large datasets is challenging due to memory constraints. While various sampling strategies exist, merging them with temporal data remains complex. Enhancing GNN's scalability for real-time applications is a critical research area~\cite{jin2023survey}.
For a comprehensive review on GNN-based approaches for time series analysis we refer the reader to the survey by~\cite{jin2023survey}.



\subsection{Low-latency methods}

\textit{APAN}~\cite{wang2021apan} proposes to reduce the latency at inference time by decoupling the more costly graph operations from the inference module. The authors propose a more light-weight inference module that computes the predictions based on a node's embedding as well as the messages recently received from interacting nodes, stored in the node's "mailbox". The mailbox is updated \textit{asynchronously}, i.e. separated from the inference module, and involves the more expensive $k$-hop message passing. While \textit{APAN} improves the latency at inference time, it sacrifices some memory since each node's state is now expanded with a mailbox, and more importantly it potentially uses outdated information at inference time due to asynchronous update of this mailbox. This algorithm addresses the need to generate low-latency embeddings, similar to our \textit{Deep-Graph-Sprints} methods. However, unlike our methods, \textit{APAN} uses outdated information which could negatively affect its overall performance.


Moreover, towards reducing computational costs of GNNs, \textit{HashGNN}~\cite{wu2021hashing} leverages MinHash (an algorithm used to efficiently estimate the similarity between sets, by hashing their elements into a smaller representative set of hash values) to generate node embeddings suitable for the link prediction task, where nodes that results in the same hashed embedding are considered similar. \textit{SGSketch}~\cite{yang2022streaming} is a streaming node embedding framework uses a mechanism to gradually forget outdated edges, achieving significant speedups. Differently than our approach \textit{SGSketch} uses the gradual forgetting strategy to update the adjacency matrix and therefore only considers the graph structure.


\cite{liu2019real} propose an algorithm for graph streams that performs node representation updates in real-time by: 1) Identifying nodes influenced by newly added nodes (e.g., one-hop neighbors); 2) Generating embeddings for new nodes through linear summation of influenced nodes' embeddings; 3) Adjusting the embeddings of these influenced nodes. Therefore generating approximated embeddings  in low latency. However, the embeddings depend only on the neighbors embeddings and ignoring the target vertex attributes.

%Graph-Sprints~\cite{eddin2023random} provide an approximation of random walks for low latency graph feature extraction...



Jiqun et. al.,~\cite{chu2024incorporating} propose Exponential Smoothing Multi-Layer Perceptron (ETSMLP) model, which leverages an exponential smoothing technique to model long-term dependencies in sequence learning. 
The model employs two learnable damped factors, to modify the influence of a smoothing factor and the current input, respectively. These factors enable the model to adjust the impact of past and current data adaptively. It treats the learnable and smoothing factors as complex numbers for a richer representation.


%While our method aligns with the memory function of the Temporal Graph Network (TGN), it diverges by addressing TGN's limitations. TGN's substantial computational and memory requirements hinder its ability to capture long-term dependencies, a concern elaborated in Section~\ref{sec:background_learning_mechanisms_modes}. Our framework stands out by optimizing resource usage and maintaining the ability to capture long-term dependencies, thus, effectively addressing the constraints associated with TGN.

==> 4-results_nc.tex <==
\section{Experiments and Results}
\label{sec:deep_graph_sprints_results}

\subsection{Experimental Setup}
\label{sec:deep_graph_sprints_experimental_setup}

The efficacy of our methodology was evaluated through the node classification task across five different datasets. This include three open-source external datasets and two proprietary datasets from the AML domain.

\subsection*{Baselines}
\label{sec:baselines}

We compare the performance of our method against several baselines.

The first simple baseline, we call \textit{Raw}, trains a machine learning model using only raw edge features.


Another baseline is \textit{Graph-Sprints}~\cite{eddin2023random} a graph feature engineering method, we refer to it by~\textit{GS}. The \textit{GS} baseline, use the same ML classifier used by the \textit{Raw} baseline but diverge in the feature used for training— GS employs \textit{Graph-Sprints} histograms, and \textit{Raw} employs the raw edge features.

%An additional baseline, termed \textit{Fixed-DGS}, represents a variant of \textit{DGS} where the DGS parameters remain static during training. The purpose of this baseline is to highlight the performance enhancement attributed to the learning of DGS parameters.



An additional baseline set comprises state-of-the-art GNN methods, specifically \textit{TGN}~\cite{tgn_icml_grl2020}. Our TGN implementation, based on PyTorch Geometric~\cite{Fey/Lenssen/2019}, differs from the original by restricting within-batch neighbor sampling. A difference between our implementation and the default PyTorch Geometric approach, which does not update the state with current edge features before classification, a common practice in link prediction tasks. To ensure a fair comparison, we incorporate edge features into the node state before classification. For consistency, \textit{GS} and \textit{DGS} also employ the same constraints.

%Another difference is that the available PyTorch Geometric implementation doesn't update the state of the node with the edge features before passing it to the classifier (which is a suitable implementation for the link prediction task). For a fair comparison with our method that utilizes this information, we update the state with the edge features before the classifier.

Several TGN variants were used:  \textit{TGN-attn}, aligning with the original paper’s robust variant, \textit{TGN-ID}, a simplified version focusing solely on memory module embeddings, and \textit{Jodie}, which utilizes a time projection embedding with gated recurrent units.  \textit{TGN-ID} and  \textit{Jodie} baselines, which do not necessitate neighbor sampling, were chosen for their lower-latency attributes compared to  \textit{TGN-attn}.

GNN baselines (\textit{TGN-ID},  \textit{TGN-attn}, and  \textit{Jodie}) all used a node embedding size of 100



\subsection*{Optimization}
\label{app:dgs_hp_ranges}

The hyperparameter optimization process utilizes Optuna~\cite{akiba2019optuna} for training 100 models. Initial 70 trials are conducted through random sampling, followed by the application of the TPE sampler. Each model incorporated an early stopping mechanism, triggered after 10 epochs without improvement. This criterion, based on the AUC, ensured efficient training. Table~\ref{tab:dgs_hpt_params} enumerates the hyperparameters and their respective ranges employed in the tuning process of  \textit{DGS} and the baselines. All represents the hyperparameters that are common to all the used methods (i.e., DGS, GS, and GNN)


\begin{table}[htb]
\centering
\caption{Hyperparameters ranges for \textbf{DGS} and baseline methods.}
%Hyperparameters ranges for the \textit{Graph-Sprints} (GS) method and the other baselines (GNN)}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Hyperparameter} & \textbf{min} & \textbf{max} \\ \hline
\textbf{DGS} & DGS learning rate (\(\eta\)) & 0.0001 & 1000 \\ \hline
\textbf{DGS} & Number of softmaxes ($x$) & 10 & 50 \\ \hline

\textbf{GS} & $\alpha$ & 0.1 & 1  \\ \hline
\textbf{GS} & $\beta$  & 0.1 & 1 \\ \hline

\textbf{GNN}  & Memory size & 32 & 256 \\ \hline
\textbf{GNN}  & Neighbors per node & 5 & 10 \\ \hline
\textbf{GNN}  & Num GNN layers & 1 & 3 \\ \hline
\textbf{GNN}  & Size GNN layer & 32 & 256 \\ \hline


\textbf{ALL}  & Learning rate &  0.0001 & 0.01 \\ \hline
\textbf{ALL}  & Dropout perc & 0.1 & 0.3 \\ \hline
\textbf{ALL}  & Weight decay & 0.000000001 & 0.001 \\ \hline
\textbf{ALL}  & Num of dense layers & 1 & 3 \\ \hline
\textbf{ALL}  & Size of dense layer &  32 & 256 \\ \hline
%\textbf{GNN/GS}  & Batch size & 128 & 2024 \\ \hline
%\textbf{GNN/GS}  & Perc of positive class & 0.1 & 0.5 \\ \hline


\end{tabular}
\label{tab:dgs_hpt_params}

\end{table}



%Importantly, for \textit{DGS}, the state size is set at 100 (i.e., number of softmaxes $\times$ number of rows per softmax=100, $x \times h = 100$), ensuring a fair comparison with other GNN baseline models (\textit{TGN-ID},  \textit{TGN-attn}, and  \textit{Jodie}). In future experiments, we propose to maintain a constant $h$ (i.e., number of rows per softmax function) while varying the number of softmaxes.

Importantly, the state size for \textit{DGS} is fixed to 100, achieved by setting the product of the number of softmax functions and the number of rows per softmax to 100 ($x \times h = 100$). This aligns with the configurations of other GNN baseline models (\textit{TGN-ID}, \textit{TGN-attn}, and \textit{Jodie}) to ensure comparability. In future experiments, one could vary the number of softmax functions while keeping the number of rows per softmax ($h$) constant.


\subsection*{Datasets}
We leverage two sets of datasets, the first one contains three publicly available datasets~\cite{kumar2019predicting} from the social and education domains. We detail their main characteristics in Table~\ref{table:external_data_stats}. All datasets are CTDGs and are labeled. Each dataset is split into train, validation, and test sets respecting time (i.e., all events in the train are older than the events in validation, and all events in validation are older than the events in the test set). In the public datasets, we adopt the identical data partitioning strategy employed by the baseline methods we compare against, which also utilized these datasets. 

The second set of datasets is from the AML domain, and contains two real-world banking datasets. Due to privacy concerns, we can not disclose the identity of the FIs nor provide exact details regarding the node features. We refer to the datasets as \textit{FI-A} and \textit{FI-B}. The graphs in this use-case are constructed by considering the accounts as nodes and the money transfers between accounts as edges.
Table~\ref{table:external_data_stats} shows the details of these datasets. 



\begin{table}[htb]
\centering
\caption{Information and data partitioning strategy for public~\cite{kumar2019predicting}, and proprietary datasets. In the public datasets, we adopt the identical data partitioning strategy employed by the baseline methods we compare against, which also utilized these datasets. In the proporitary datasets(FI-A, FI-B) due to privacy concetraints we provide approximated details}
\begin{tabular}{|c|c|c|c||c|c|}
\hline
\textbf{}  & \textbf{Wikipedia} & \textbf{Mooc} & \textbf{Reddit} & \textbf{FI-A} & \textbf{FI-B} \\ \hline
\#Nodes & 9,227 & 7,047 & 10,984 & $\approx$400,000 & $\approx$10,000 \\ \hline
\#Edges & 157,474 &  411,749 & 672,447 & $\approx$500,000 & $\approx$2,000,000 \\ \hline
Label type & editing ban &  student drop-out & posting ban & AML SAR & AML escalation \\ \hline
Positive labels & 0.14\% &  0.98\%  & 0.05\% & 2-5\% & 20-40\% \\ \hline
Duration & 30 days & 29 days & 30 days & $\approx$300 days  &  $\approx$600 days \\ \hline
%Edges/day (mean ± std)  & & & &  1500 ± 750  & 3000 ± 5000 \\ \hline
%Used split & 75\%-15\%-15\% & 60\%-20\%-20\% & 75\%-15\%-15\%  &  60\%-10\%-30\%  & 60\%-10\%-30\% \\ \hline
Used split (\%) & 75-15-15 & 60-20-20 & 75-15-15  &  60-10-30  & 60-10-30 \\ \hline

\end{tabular}
\label{table:external_data_stats}
\end{table}


%\begin{table}[ht]
%\centering
%\caption{Information and data partitioning strategy for AML datasets.}
%\begin{tabular}{|c|c|c|}
%\hline
%\textbf{} & \textbf{FI-A} & \textbf{FI-B} \\ \hline
%\#Nodes & $\approx$400000 & $\approx$10000  \\ \hline
%\#Edges & $\approx$500000 & $\approx$2000000  \\ \hline
%Positive labels & 2-5\% & 20-40\% \\ \hline
%Duration &  $\approx$300 days  &  $\approx$600 days \\ \hline
%Edges/day (mean ± std)  &  1500 ± 750  & 3000 ± 5000 \\ \hline
%Used split &  60\%-10\%-30\%  & 60\%-10\%-30\% \\ \hline
%\end{tabular}
%\label{table:internal_data_stats}
%\end{table}



\subsection{Node classification} 
\label{subsec: deep_graph_sprints_results_node_classification}

The results for \textbf{node classification} are detailed in Table~\ref{table:dgs_results_external_data_nc}, displaying the average test AUC ± std for the external datasets and the $\Delta$ AUC for the AML datasets. To obtain these figures, we retrained the best model identified through hyperparameter optimization across 10 different random seeds. 

%\textit{DGS} along with the GNN baselines (\textit{TGN-ID},  \textit{TGN-attn}, and  \textit{Jodie}) all utilized the same embedding size of 100.

We have highlighted the \textbf{best} and \underline{second-best} performing models for each dataset. To provide an overview, we include a column showing the average rank, representing the mean ranking computed from all datasets. Remarkably, \textit{DGS} achieves either the highest or the second-highest scores in four out of the five datasets. The exception is the Mooc dataset, where GNN baselines surpass our method. It is crucial to note that these GNN baselines appear to be overfitting the validation split. When evaluated without leveraging the latest edge features, their performance improved, indicating reduced overfitting.

%\textit{DGS} performed exceptionally well in the Wikipedia and Mooc datasets, achieving the highest scores, while \textit{Graph-Sprints} performed the second-best. In the Reddit dataset, our methods ranked second, behind \textit{Graph-Sprints}. 
%To provide an overview, we include a column showing the average rank, in Table~\ref{table:dgs_results_external_data_nc},  which represents the mean ranking computed from all datasets.



%The lower performance of DGS in the Wikipedia dataset, compared to other \textit{DGS} variations, is noteworthy. Initial analysis indicates that this is due to the data preprocessing method for the Wikipedia dataset. While using a consistent standardization approach across all datasets, omitting this step improved DGS-3's performance to $89.2 \pm 1.9$. Nonetheless, for consistency in the results table, the performance with standard preprocessing is reported.  Future research will focus on understanding and resolving the factors behind this difference in DGS-3's performance.


\begin{table}[htb]
\centering
\caption{Node classification results using public and internal datasets.}
\begin{tabular}{|c|c|c|c||c|c|c|}
\hline
\multirow{2}{*}{\textbf{Method}} &\multicolumn{3}{|c||}{\textbf{AUC ± std}} &\multicolumn{2}{|c|}{$\Delta$\textbf{AUC ± std}} & \multirow{2}{*}{\parbox{1.25cm}{\raggedright\textbf{Average \\ rank}}} \\ \cline{2-6}

  & \textbf{Wikipedia} & \textbf{Mooc} & \textbf{Reddit} & \textbf{FI-A} & \textbf{FI-B} & \\ \hline
 
 Raw & 58.5 {\tiny± 2.2} & 62.8 {\tiny± 0.9} & 55.3 {\tiny± 0.8}  & 0 & 0 &  6 \\ \hline
 
% Fixed-DGS  & 87.3 ± 1.7 & 72.7 ± 0.3 &  64.5 ± 0.4  &  6.3  \\ \hline 
 
 TGN-ID  & 69.3{\tiny ± 0.5} & \textbf{86.3{\tiny ± 0.8}} & 56.2 {\tiny± 3.7} &  +1.2 {\tiny± 0.1} & +24.3 {\tiny± 1.8} &  3.4   \\ \hline
 
 
 Jodie   & 68.8 {\tiny± 1.3} & \underline{86.1 {\tiny± 0.4}} & 56.2 {\tiny± 2.1} &  +1.4 {\tiny± 0.1} & +25.0 {\tiny± 0.6}  &  3.2  \\ \hline
 
 TGN-attn & 70.5 {\tiny± 4.1} & 86.0 {\tiny± 0.9} & 55.6 {\tiny± 6.1} &  +0.9 {\tiny± 0.2} & +22.5 {\tiny± 2.5} &  4.2  \\ \hline
 
 GS & \textbf{90.7 {\tiny± 0.3}} & 75.0 {\tiny± 0.2} & \textbf{68.5 {\tiny± 1.0}} &  \underline{+1.8 {\tiny± 0.5}} & \textbf{+27.8 {\tiny± 0.4}}  &  2    \\ \hline 
 DGS  & \underline{89.2 {\tiny± 2.2}} & 78.7 {\tiny± 0.6} & \underline{68.0 {\tiny± 1.9}} & \textbf{+3.6 {\tiny± 0.2}}  & \underline{+26.9 {\tiny± 0.3}}  &  2.2    \\ \hline 

\end{tabular}
\label{table:dgs_results_external_data_nc}
\end{table}





\subsection{Inference Runtime} 

\textit{DGS} has a primary goal of achieving reduced inference times. Comparative latency assessments were conducted amongst \textit{DGS}, \textit{Graph-Sprints}, and baseline GNN models. These assessments entailed processing 200 batches, each containing 200 events, across distinct datasets (Wikipedia, Mooc, and Reddit) for node classification task. The average times were computed over 10 iterations. Tests were performed on a Linux PC equipped with 24 Intel Xeon CPU cores (3.70GHz) and an NVIDIA GeForce RTX 2080 Ti GPU (11GB). 


As depicted in Figure~\ref{fig:deep_graph_sprints_results_run_time_auc}, \textit{DGS} exhibited significant speed advantages. On the Reddit dataset, it was more than tenfold faster than the \textit{TGN} GNN baseline. For the smaller datasets, this speed enhancement ranged approximately between 5 and 6 times. Notably, the runtime of \textit{DGS} remained stable and was not influenced by the graph's edge count. This stability suggests that speed gains may be more pronounced in larger graphs, especially considering that inference times in the \textit{TGN} approach are impacted by the number of graph edges. Moreover, 
When benchmarked against other GNNs baselines (\textit{TGN-ID}, \textit{Jodie}), \textit{DGS} consistently demonstrated significantly lower inference latency. 

In comparison to the \textit{Graph-Sprints} framework, known for its low latency, \textit{DGS} generally exhibited marginally superior speed, especially noticeable in the Wikipedia and Reddit datasets, with latencies of 0.24 versus 0.29 seconds. This performance gain can be attributed to the higher feature count in these datasets (172 features), which potentially increases the processing time for \textit{Graph-Sprints} due to the elevated feature volume. In contrast, for the Mooc dataset, which has only 7 edge features, \textit{Graph-Sprints} showed a slight edge in speed (0.24 versus 0.28 seconds).




\begin{figure*}[htb]
\center
\includegraphics[width=\textwidth]{Figures/dgs_speedups_nc_2.png}
\caption{Trade-off between AUC and runtime.}
\label{fig:deep_graph_sprints_results_run_time_auc}
\end{figure*}


\subsection{Ablation Study}
This section delineates a comparative analysis of three distinct variants of the \textit{DGS} methodology, differentiated primarily by their parameterization complexity.

The initial variant, designated as \textit{DGS-s}, constitutes the most basic approach wherein \textit{scalar} parameters $\alpha$ and $\beta$ are learned. Moreover, instead of employing a learnable embedding matrix, \textit{DGS-s} adopts the static embedding function utilized by \textit{Graph-Sprints}.


The subsequent variant, \textit{DGS-v}, retains the fixed embedding function but transitions to \textit{vectorized} parameters, $\vec{\alpha}$ and $\vec{\beta}$. This modification is intended to explore the effects of enhancing the parameter complexity on the performance of the model.

The final variant, the principal model described herein as \textit{DGS}, not only incorporates \textit{vectorized} parameters $\vec{\alpha}$ and $\vec{\beta}$ but also integrates a learnable embedding matrix. This comprehensive approach aims to assess the impact of maximal parameter flexibility on the model's efficacy.

Table~\ref{table:dgs_results_external_data_nc_ablation_study} presents the results of the three variants for \textbf{node classification} across five different datasets. It displays the average test AUC ± standard deviation for the external datasets and the $\Delta$ AUC for the AML datasets.

\begin{table}[htb]
\centering
\caption{\textit{DGS:} Ablation study, Node classification results}
\begin{tabular}{|c|c|c|c||c|c|c|}
\hline
\multirow{2}{*}{\textbf{Method}} &\multicolumn{3}{|c||}{\textbf{AUC ± std}} &\multicolumn{2}{|c|}{$\Delta$\textbf{AUC ± std}} & \multirow{2}{*}{\parbox{1.25cm}{\raggedright\textbf{Average \\ rank}}} \\ \cline{2-6}

  & \textbf{Wikipedia} & \textbf{Mooc} & \textbf{Reddit} & \textbf{FI-A} & \textbf{FI-B} & \\ \hline
 
 DGS-s   & 88.2 {\tiny± 0.6} & 73.8 {\tiny± 0.5} & 65.8 {\tiny± 0.8} &  +1.8 {\tiny± 0.3} & 25.8 {\tiny± 0.7}  &  3  \\ \hline
 
 DGS-v & \textbf{91.0 {\tiny± 0.3}} & 75.2 {\tiny± 0.3} & 67.2 {\tiny± 0.4} &  +3.2 {\tiny± 0.1} & +26.7 {\tiny± 0.2} &  1.8  \\ \hline
 
 DGS  & 89.2 {\tiny± 2.2} & \textbf{78.7 {\tiny± 0.6}} & \textbf{68.0 {\tiny± 1.9}} & \textbf{+3.6 {\tiny± 0.2}}  & \textbf{+26.9 {\tiny± 0.3}}  &  1.2    \\ \hline 

\end{tabular}
\label{table:dgs_results_external_data_nc_ablation_study}
\end{table}





==> 6-future_work.tex <==


\section{Future Work}
\label{sec:deep_graph_sprints_future_work}

In the previous sections we proposed the \textit{DGS} method, with certain decisions, however many of the options can be adapted to further enhance the method.



\subsection*{Exploration of Various Standardization Functions}

In the conducted experiments, the softmax function was utilized to ensure that the cumulative sum of all elements within a single embedded feature is equal to one, with each individual element ranging from 0 to 1. The investigation of alternative standardization methods will be addressed in future research.

\subsection*{Advanced Optimization Techniques:}
The incorporation of an advanced optimization algorithms such as Adam could potentially replace the current use of stochastic gradient descent in updating the DGS parameters during forward-mode AD. The adoption of these advanced techniques is anticipated to facilitate the learning of optimal parameters and therefore more easily achieving good performance.
%enhance convergence rates and reinforce model robustness, thereby elevating the overall efficiency of the method.


\subsection*{Extension to Heterogeneous Graphs:}
A significant area of future research for the \textit{DGS} method is its adaptation to heterogeneous graph structures. This evolution aims to extend the method's applicability across a diverse array of graph-based problem domains. One viable approach is to employ distinct embedding matrices for different node or edge types, where each matrix maps varied input features to a consistent embedding dimension. This method, however, presents challenges in mini-batch training, necessitating the segregation of edges by type for effective mapping.

An alternative approach involves implementing a unique update process for each node or edge type, resulting in the creation of multiple sub-embeddings. These sub-embeddings would then be concatenated to form a unified final embedding. The key consideration here is determining whether to learn a singular embedding matrix \( W \) per node or edge type, or to learn a complete set of parameters — \( \vec{\alpha}, \vec{\beta}, \) and \( W \) — for each type. The decision on this architecture is likely to be dependent on the use cases.

Central to this adaptation is that the structure of the model needs to be defined, after which the parameters are learned autonomously during training, obviating the need for manual adjustments as required in \textit{Graph-Sprints}.



\subsection*{Input-Dependent Parameters:}
A significant enhancement under consideration involves enabling input-dependent adaptability for the parameters alpha (\(\vec{\alpha}\)) and beta (\(\vec{\beta}\)). This advancement aims to amplify the model's responsiveness to diverse data inputs. As such, the state update equation would undergo modification, integrating trainable matrices \( W_1, \) and \( W_2 \) of dimension \( (s \times f) \), where \( s \) represents the embedding size and \( f \) denotes the number of input features. 

To ensure the parameter values remain within the range [0, 1], a sigmoid function per feature, denoted as \( \psi \), can be employed. The parameters are thus defined as:
\[ \vec{\alpha} = \psi(W_1 F_t), \]
and 
\[ \vec{\beta} = \psi(W_2 F_t). \]

The revised state update formula, encapsulated in Equation~\ref{eq:deep_graph_sprints_4_input_dependent}, effectively integrates these changes:

\begin{equation}
\vec{S}_t = \psi(W_2 F_t) \odot S_{t-1} + (1 - \psi(W_2 F_t)) \odot \left((1 - \psi(W_1 F_t)) \odot \vec{\sigma}(W F_t) + \psi(W_1 F_t) \odot \vec{S}^*_{t-1}\right)
\label{eq:deep_graph_sprints_4_input_dependent}
\end{equation}

This modification enhances the accuracy of the \textit{DGS} model in processing varying inputs.



These future directions represent critical steps towards augmenting the sophistication and versatility of the \textit{DGS} model, positioning it at the forefront of graph representation learning tools.
